Pool of Experts: Realtime Querying Specialized Knowledge in Massive Neural Networks

In spite of the great success of deep learning technologies, training and delivery of a practically serviceable model is still a highly time-consuming process. Furthermore, a resulting model is usually too generic and heavyweight, and hence essentially goes through another expensive model compression phase to fit in a resource-limited device like embedded systems. Inspired by the fact that a machine learning task specifically requested by mobile users is often much simpler than it is supported by a massive generic model, this paper proposes a framework, called Pool of Experts (PoE), that instantly builds a lightweight and task-specific model without any training process. For a realtime model querying service, PoE first extracts a pool of primitive components, called experts, from a well-trained and sufficiently generic network by exploiting a novel conditional knowledge distillation method, and then performs our train-free knowledge consolidation to quickly combine necessary experts into a lightweight network for a target task. Thanks to this train-free property, in our thorough empirical study, PoE can build a fairly accurate yet compact model in a realtime manner, whereas it takes a few minutes per query for the other training methods to achieve a similar level of the accuracy.

==> coverletter.tex <==
\twocolumn


We highly appreciate the valuable feedback of the reviewers. We have used the comments to considerably improve the quality of our paper. Major changes are summarized as follows:
\begin{itemize}
    \item We have strengthened and clarified our target scenario by adding and revising several sentences in the introduction. In particular, we focus on the space-efficiency of our PoE framework, which is newly founded thanks to Reviewer 1.
    \item We have re-conducted all the experiments in order to test more different combinations and to show more distributional information like standard deviation along with average.
    \item We have newly conducted a thorough empirical study on the performance comparison between $L_{soft}$ and $L_{scale}$, where the corresponding experimental results have been added at the end of Section \ref{sec:experiments:service}.
    \item We attempted to make the overall presentation better and added supplementary descriptions in many parts of the paper for a clearer understanding of the content in response to the reviewers' comments.
    \item Due to the space limitation, some new detailed experimental results are presented in our anonymized github page\footnote{\url{https://github.com/PoE-code/Pool-of-Experts-code}}, to which we have made another major revision. 
\end{itemize}
Below, we answer the questions that have been raised, and clarify how the reviewers' concerns have been addressed in the revised version. In the paper, we highlight major changes in \add{blue color}, which will be back to black in the final CRC version.

\section*{Reviewer 1}
\smalltitle{Comment (O1)}
The motivation application is not convincing. As long as we know $Q$ (e.g., recognizing images from a zoo or images from a restaurant) in advance, we can always pretrain a lightweight model or compress a big model to serve the requests accurately and efficiently. If we do not know $Q$, then we would not know which expert models to select. When do we really need to create a new model by combining a pool of expert models? Can you give a concrete scenario?

My point is no matter what the application scenario is, the expert model has to be trained. After training the expert models (for an animal theme park), the service provider can also train a lightweight or compressed generic model. Then the requests can be handled when then users visit the park. Is there any scenario that this approach does not work? What is the issue of this approach (note that the compressed ML model is trained by the same developer for the expert model).

\smalltitle{Response (O1)}
We understand what the reviewer concerns on the application of this work. As mentioned in our first author feedback, this work is intended for a scalable AI-as-a-Service (AIaaS) scenario, where there exist multiple users (at the same time or who probably are non-experts). Our point here is that we cannot fully expect which user requests which form of $Q$ in advance as a service provider like Google cannot know which keyword will be queried in advance and hence cannot pre-build all the possible search results. Likewise, we cannot train and compress the complete set of specialized models for all the possible combinations of primitive tasks (i.e., $2^n$, where $n$ is the number of all the primitive tasks). As the reviewer pointed out in A1, this approach requires a huge amount of storage for maintaining all $2^n$ lightweight models with high preprocessing overhead. As shown in Table \ref{tab:Volumes} newly added in this version, our PoE takes much less storage to instantly build a specialized model for any of all $2^n$ combinations of tasks.

Please refer to all the changes in the introduction and Table \ref{tab:Volumes} to clarify our target scenario.


\thispagestyle{empty}

\smalltitle{Comment (O2)}
(a) There is no analysis for the results in Table 2. For example, why is CKD better than transfer learning? Note that for the task of Table 2, transfer learning has no issues of overconfident experts and logit scale. (b) What is the hyper-parameter settings for the baseline models, e.g., the total number of epochs? Have you tuned these hyper-parameters? The provided code does not include the baseline algorithms.

\smalltitle{Response (O2)}
(a) We have added analysis about comparison between CKD and Transfer in Section \ref{sec:experiment:special}. (b) In our current github page, we have fully described all the hyperparameters, and included all the baseline algorithms. Also, in the paper, we have newly mentioned important hyperparameter values such as $\alpha = 0.3$. 

\smalltitle{Comment (O3)}
Why not compare the proposed solution with model compression techniques[1], e.g., quantization methods, which give a small and generic model? It would be better to include a subsection in the related work to discuss the difference to quantization methods in terms of the application scenario. If they can be applied in the same applications, then it is necessary to do some experimental comparison.

\smalltitle{Response (O3)}
As mentioned in our first rebuttal, three major schemes on neural network compression, namely knowledge distillation, quantization, and network pruning, are complementary to each other, and quantization does not actually reduce the number of FLOPs (and params), which makes difficult for quantization to fairly compare with knowledge distillation. However, in response to the reviewer's comment, we have expanded the subtopic `knowledge distillation' to `neural network compression' in Section \ref{sec:related} so that we can incorporate representative methods on quantization and network pruning.


\smalltitle{Comment (A1)}
For the proposed solution, we need to maintain a pool of expert models. Will the total storage of the pool be very large? Is there any comparison in terms of this storage cost?

\smalltitle{Response (A1)}
As mentioned in our first feedback, the total size of PoE is 20-30 times smaller than those of oracle themselves. More importantly, we have newly included the total estimated volume of the complete set of specialized models for all the possible combinations of primitive tasks. Even though we assume that every specialized model has the same size as the minimum expert, the total estimated volumes of those complete sets would be extremely larger (e.g., 1198.40 TB for Tiny-ImageNet) than those of PoE (e.g., 3.20 MB for Tiny-ImageNet), as shown in Table \ref{tab:Volumes}.



\section*{Reviewer 2}
\smalltitle{Comment (O1)}
It would be great if the authors can provide more empirical results about the difference of training with $L_{scale}$ and $L_{soft}$.

\smalltitle{Response (O1)}
According to the reviewer's comment, we have conducted a thorough empirical study to see how the result can be changed when using either of $L_{scale}$ or $L_{soft}$ alone. In summary, $L_{soft}$ turns out to be better than $L_{scale}$ at transferring the oracle's knowledge, whereas $L_{scale}$ is still more useful than $L_{soft}$ when addressing the logit scale problem, as we expected. Please refer to the corresponding experimental results and descriptions of Table \ref{tab:soft and scale}. 

Considering this new experimental result summarized in Table \ref{tab:soft and scale} and the strict space limitation, we had to exclude a more detailed analysis solely focused on the effectiveness of $\L_{scale}$, which was originally included in our first version and has not been changed ever since. For all the experimental results excluded in this revised paper, please refer to our github page.

\smalltitle{Comment (D3)}
From the experiments, it is not clear what limitations the proposed method has.
It would be great if the authors can try different combinations for the same $n(Q)$ and report the tale and more distributional information.

\smalltitle{Response (D3)}
According to the reviewer's comment, in this version, we re-conducted all the experiments for Tables \ref{tab:specialized result}, \ref{tab:merge test} and \ref{tab:soft and scale}, where we present the average over 6 different combinations with the same $n(Q)$. Moreover, we have additionally included the standard deviation for each average accuracy in all those tables, which does not seem to contradict to the overall trend of experimental results.

\smalltitle{Comment (D4)}
I feel that the dataset used in this work is a little bit small for a simple (which is a good thing) method like this.

\smalltitle{Response (D4)}
As we mentioned in our first feedback, we are working on building a more practical version of PoE trained on the full ImageNet dataset, whose experimental results are being released in our github page.

Unfortunately, we decided not to test all our competitors (e.g., Scratch, Transfer, SD, UHC, etc.) with ImageNet, as most of them, unlike our PoE, require a heavy training process to the point that it takes at least several days for each competitor to test only one training configuration. We indeed believe that the current experimental results using CIFAR-100 and Tiny-ImageNet well justify the fact that our PoE outperforms its competitors in both accuracy and efficiency. 

Please refer to our github page for our current experimental results of PoE with the full ImageNet dataset.


\section*{Reviewer 3}
\smalltitle{Comment}
The notation ($\times$ 43 $\downarrow$) used in a lot of the tables is a bit confusing; it's not obvious what this means at first glance.
\smalltitle{Response} The notation $\times$ 43 $\downarrow$ actually means the corresponding value (e.g., the size of specialized model) gets 43 times smaller than its original value (e.g., the size of oracle). Agreeing with the reviewer, we have accordingly changed all occurrences of $\times~xx \downarrow$ like to be $\times \frac{1}{xx}$. Please refer to Tables \ref{tab:specialized result} and \ref{tab:merge test}.


\smalltitle{Comment}
The paper would be stronger if we had a more concrete example of what sort of task this would be useful for. Why would we need a realtime model querying system?

\smalltitle{Response}
Thank you very much for the positive feedback. We hope you to like the new version even more because we have further clarified the target scenario of our work in the introduction and conducted new experiments. The necessity of a realtime model querying system would be to maintain the quality of service if we really have such an AIaaS system that should provide any on-demand tiny models requested by multiple users. Even though this paper focuses on the task of image classification as a first proposal, we can think of any task that can be decomposed into multiple sub-tasks, e.g., specific domains, specific dimensions, etc.

\onecolumn
% \newpage
